Sanity Check for External Clustering Validation Benchmarks using Internal Validation Measures

We address the lack of reliability in benchmarking clustering techniques based on labeled datasets. A standard scheme in external clustering validation is to use class labels as ground truth clusters, based on the assumption that each class forms a single, clearly separated cluster. However, as such cluster-label matching (CLM) assumption often breaks, the lack of conducting a sanity check for the CLM of benchmark datasets casts doubt on the validity of external validations. Still, evaluating the degree of CLM is challenging. For example, internal clustering validation measures can be used to quantify CLM within the same dataset to evaluate its different clusterings but are not designed to compare clusterings of different datasets. In this work, we propose a principled way to generate between-dataset internal measures that enable the comparison of CLM across datasets. We first determine four axioms for between-dataset internal measures, complementing Ackerman and Ben-David's within-dataset axioms. We then propose processes to generalize internal measures to fulfill these new axioms, and use them to extend the widely used Calinski-Harabasz index for between-dataset CLM evaluation. Through quantitative experiments, we (1) verify the validity and necessity of the generalization processes and (2) show that the proposed between-dataset Calinski-Harabasz index accurately evaluates CLM across datasets. Finally, we demonstrate the importance of evaluating CLM of benchmark datasets before conducting external validation.

==> appendices/A_within_axioms.tex <==
\section{Detailed Description of \textit{Within-Dataset} Axioms}

\label{app:within}


% \mac{Put all that material in appendix, keep only one paragraph summarizing the four axioms. Michael: Double-check there is no error in reproducing the definitions and their interpretation. Let us name within-axioms W1, W2... and our new between-axioms B1, B2...}

% The first within-dataset axiom requires the measures to be invariant against the change of scale.

\textbf{(Axiom W1) \textit{Scale Invariance.} } \textit{A measure $f$ satisfies scale invariance if $\forall X$, $ \forall d$, $\forall C$ over $(X, d)$, $f(C, X, d) = f(C, X, \alpha d)$ $\forall \alpha > 0$ (where  $\alpha d$ is a distance function satisfying $\alpha d(x,y) = \alpha \cdot d(x,y)$, $ \forall x, y \in X$) }


% The second axiom asks whether a measure is consistent, which means its value increases when the contrast between within-compactness and between-separability of the classes gets bigger. \

% In other words, $d'$ has smaller within-cluster distance and bigger between-cluster distance compared to $d$ over $C$. Then, the axiom is defined as:

\textbf{$C$-consistent variant.} $d'$ is a $C$-consistent variant of $d$ if $d'(x, y) \leq d(x,y)$ implies $x \sim_C y$, and $d'(x, y) \geq d(x,y)$ implies $ x \nsim_C y$


\textbf{(Axiom W2) \textit{Consistency.} } \textit{A measure $f$ satisfies consistency if  $\forall X$, $ \forall d$, $\forall C$ over $(X, d)$, whenever $d'$ is a $C$-consistent variant of $d$, $f(C, X, d') \geq f(C, X, d)$.}


% The third axiom requires the measures to be rich; any clustering should have an opportunity to have a best score over the domain by modifying the distance function. 

\textbf{(Axiom W3) \textit{Richness. }} \textit{A measure $f$ satisfies richness if $\forall X$, $\forall C$ over $X$, there exists $d$ over $X$ such that $C = \arg\max_{C_i \in \mathcal{C}}f(C_i, X, d)$ (where  $\mathcal{C}$ denotes the set of all possible clusterings over $X$)}

% The last axiom is added to prevent a function that consider the identity of domain points (e.g., relate class labels to the score) to be regarded as a within-dataset internal measure.

\textbf{Clustering Isomorphism. } \textit{Two clustering $C, C'$ over $(X, d)$ are isomorphic (i.e., $C \approx_d C' $), if there exists distance-preserving isomorphism $\phi: X \rightarrow X$, such that $\forall x, y \in X$, $x \sim_C y$ if and only if $\phi(x) \sim_{C'} \phi(y)$.} 

\textbf{(Axiom W4) \textit{Isomorphism Invariance}.} \textit{A measure $f$ satisfies isomorphism invariance if $\forall X$, $ \forall d$, $\forall C, C'$ where $C \approx_d C'$, $f(C, X, d) = f(C', X, d)$. } 



==> appendices/B_theorem_proof.tex <==
\section{Theorems and Proofs}

\subsection{About Calinski-Harabasz Index ($CH$) and Axioms}


% \mac{CH index is not mention in Miligan paper which is cited in BenDavid for studying techniques that all verify Within datasets axioms. So here we prove that CH verify the within-datasets axioms. Therefore CHbtwn also verify these axioms.}



\textbf{Theorem 1.} \textit{Calinski-Harabasz Index ($CH$) satisfies Scale Invariance.}

\textit{Proof. } Consider $C$ over $(X, d)$, and assume that $d'$ be a distance function satisfying $d' = \alpha d(x,y)$ for $\alpha > 0$. Then, 
\[
CH(C, X, d') =  \frac{\sum_{i=1}^{|C|}|C_i|\alpha^2 d^2(c_i, c) / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} \alpha^2  d^2(x, c_i) / (|X| - |C|)} = \frac{ \alpha ^2}{\alpha^2 } CH(C, X, d) = CH(C, X, d).
\]
Therefore, $CH$ is scale-invariant. \hfill $\Box$

% \textbf{Theorem 2.} \textit{$CH$ satisfies Consistency.}

% \textit{Proof. } Consider $C$ over $(X, d)$, and assume that $d'$ is a $C$-consistent variant of $d$. 

% For denominator, $\sum_{x\in C_i} d^2(x, c_i) = \frac{1}{|C_i|} \sum_{(x, y) \in C_i} d^2(x,y) $  \cite{apostol03amm} (equation 6'). As $d'(x,y) \leq d(x,y)$ for $ (x,y) \in C_i$, 
% \[
% \frac{1}{|C_i|} \sum_{(x, y) \in C_i} d'^2(x,y) \leq \frac{1}{|C_i|} \sum_{(x, y) \in C_i} d^2(x,y),
% \]
% and this implies 
% \[
% \sum_{x\in C_i} d'^2(x, c_i) \leq \sum_{x\in C_i} d^2(x, c_i).
% \]

% For numerator, 
% \[
% d^2(c_i, c_j) =  \frac{1}{|C_i|\cdot |C_j|} \sum_{x \in C_i, y \in C_j}d^2(x, y) - \frac{1}{|C_i|^2} \sum_{(x,y) \in C_i} d^2(x,y) - \frac{1}{|C_j|^2} \sum_{(x,y) \in C_j} d^2(x,y)
% \]
% \cite{apostol03amm} (equation 28). As $d'(x,y) \geq d(x,y)$ for $x \sim_C y$ and $d'(x,y) \leq d(x,y)$ for $x \nsim_C y$, $d'^2(c_i, c_j) \geq d^2(c_i, c_j)$.   Since $c$ is also a centroid of $X$,  $d'^2(c_i, c) \geq d^2(c_i, c)$ for all $c_i$. 

% As the denominator of $CH(C, X, d')$ is always smaller than the one of $CH(C, X, d)$ and the numerator of $CH(C, X, d')$ is always bigger than the one of $CH(C, X, d)$, $CH(C, X, d') \geq CH(C, X, d)$. Therefore, $CH$ is consistent.

\textbf{Theorem 2.} \textit{$CH$ satisfies Richness.}

\textit{Proof. } Let $C$ be a clustering over $X$. Consider $d$ in which satisfies four conditions: (1) $d(c_i,c)=10$ where $c_i$ is a centroid of a cluster within $C$ (2) $d(c'_i,c)=1$ where $c'_i$ is a centroid of a cluster within any other possible clusterings except $C$ (3) $d(x, c_i)=1$ where $c_i$ is a centroid of a cluster within $C$ and $x$ is a member of that cluster (4) $d(x', c'_i)=10$ where $c'_i$ is a cluster within any other possible clusterings except $C$ and $x'$ is a member of that cluster. Then, $C = \arg\max_{C \in \mathcal{C}} f(C, X, d)$ where $\mathcal{C}$ is a set of all possible clusterings. \hfill $\Box$

\textbf{Theorem 3.} \textit{$CH$ satisfies Isomorphism Invariance. }

\textit{Proof. } $CH$ only considers the distances between data points, and does not regards their external identities. Therefore, for two isomorphic clustering ($C \approx_d C')$, $CH(C,X,d) = CH(C', X, d)$. \hfill $\Box$


\textbf{Theorem 4}. \textit{$CH$ does not satisfy Shift Invariance. }

\textit{Proof. } 
Consider a clustering $C$ over $(X, d)$. Then, as 
\[
CH(C, X, d + \beta) = \frac{\sum_{i=1}^{|C|}|C_i|(d(c_i, c) + \beta)^2 / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} (d(x, c_i)+\beta)^2 / (|X| - |C|)} \neq CH(C, X, d),
\]
$CH$ does not satisfy Shift Invariance.
\hfill $\Box$

\textbf{Theorem 5}. \textit{$CH$ does not satisfy Class-Cardinality Invariance.}

\textit{Proof.} $CH$ handles entire clusters within $C$ at once, rather than handling them in pairwise. Therefore, $CH$ does not satisfy Class-Cardinality Invariance.    \hfill $\Box$

\textbf{Theorem 6.} \textit{$CH$ does not satisfy Range Invariance.}

\textit{Proof. } The range of $CH$ is $(0, +\infty)$. Therefore, $CH$ is not range invariant.  \hfill $\Box$



\subsection{About Class-Cardinality Invariance}

Ackerman and Ben-David \cite{bendavid08nips} showed that if a function $f'$ satisfies within-dataset axioms, then its aggregation $f(C, X, d)  = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d)$ also satisfies the axioms. 

\textbf{Theorem 7.} \textit{If $f'$ satisfies a within-dataset axiom, then $f(C, X, d)  = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d)$ also satisfies the axiom.} \cite{bendavid08nips}



Here, we provide a proof for between-dataset axioms. 

\textbf{Theorem 8.} \textit{If $f'$ satisfies Data-Cardinality Invariance, then $f(C, X, d)  = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d)$ is also Data-Cardinality Invariance.}

\textit{Proof.} $f(C, X, d) = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d) = \text{agg}_{S \subseteq C, |S = 2|} f'(\underline{S}_\alpha, \underline{X}_\alpha, d) = f(\underline{C}_\alpha, \underline{X}_\alpha, d)$. Thus, $f$ satisfies Data-Cardinality Invariance. \hfill $\Box$

\textbf{Theorem 9.} \textit{If $f'$ satisfies Shift Invariance, then $f(C, X, d)  = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d)$ is also Shift Invariance.}

\textit{Proof.} $f(C, X, d) = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d) = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d + \beta) = f(C, X, d + \beta)$. Thus, $f$ satisfies Shift Invariance. 

\textbf{Theorem 10.} \textit{If $f'$ satisfies Range Invariance, then $f(C, X, d)  = \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d)$ is also Range Invariance.}

\textit{Proof.} $\min_C f'(C, X, d) = 0$ implies $\min_C f(C, X, d) = \min_C \text{agg}_{S \subseteq C, |S = 2|} f'(S, X, d) = 0$. In the same way, $\max_C f'(C, X, d) = 1$ implies $\max_C f(C,X, d) = 1$. Thus, $f$ is Range Invariance.


\subsection{About Between-Dataset Calinski-Harabasz Index ($CH_{btwn}$) and Axioms}


\textbf{Theorem 11.} \textit{$CH_{btwn}$ satisfies Class-Cardinality Invariance.}

\textit{Proof.} By definition, $CH_{btwn}$ is an aggregation of $CH_3$. \hfill $\Box$

\textbf{Theorem 12.} \textit{$CH_{btwn}$ satisfies Scale Invariance.}

\textit{Proof. } Consider $C$ over $(X, d)$.
\begin{multline*}
    CH_1(C, X, \alpha d ) = 
\frac{\sum_{i=1}^{|C|}|C_i|e^{(\alpha \cdot d(c_i, c)) / \sigma_{\alpha d}} / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} e^{(\alpha \cdot d(x, c_i))  / \sigma_{\alpha d }} / (|X| - |C|)} \\ 
= 
\frac{\sum_{i=1}^{|C|}|C_i|e^{(\alpha \cdot d(c_i, c)) / (\alpha \cdot \sigma_{d})} / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} e^{(\alpha \cdot d(x, c_i))  / (\alpha \cdot \sigma_{d })} / (|X| - |C|)} = CH_1(C, X, d).
\end{multline*}
Therefore, $CH_1$ is scale invariant, and this makes $CH_2$ and $CH_3$, which are the functions that gets $CH_1$ as input, Scale Invariant. Then, as $CH_{btwn}$ is an aggregation of $CH_3$, due to Theorem 7, $CH_{btwn}$ is Scale Invariant. \hfill $\Box$

% \textbf{Theorem 14.} \textit{$CH_{btwn}$ satisfies Consistency.}

% \textif{Proof.} Consider $C$ over $(X, d)$, and assume that $d'$ is a $C$-consistent variant of $d$. 

% In the proof of Theorem 2, we verified $\sum_$ and $d'^2(c_i, c) \geq d^2(c_i,c)$ 

\textbf{Theorem 13. } \textit{$CH_{btwn}$ satisfies Richness}. 

\textit{Proof.} Consider the same $C, X$, and $d$ with the proof of Theorem 2. In the case, $C = \arg\max_{C \in \mathcal{C}} CH_{btwn}(C, X, d)$ where $\mathcal{C}$ is a set of all possible clusterings. \hfill $\Box$

\textbf{Theorem 14.} \textit{$CH_{btwn}$ satisfies Isomorphism Invariance.} 

\textit{Proof.} As $CH$ is, $CH_{btwn} $ only considers the distances between data points, and does not regards their external identities. Therefore, for two isomorphic clustering ($C \approx_d C')$, $CH_{btwn}(C,X,d) = CH_{btwn}(C', X, d)$. \hfill $\Box$



\textbf{Theorem 15.} \textit{$CH_{btwn}$ satisfies Shift Invariance. }

\textit{Proof.} 
\begin{multline*}
    CH_1(C, X, d + \beta) = 
\frac{\sum_{i=1}^{|C|}|C_i|e^{(d(c_i, c) + \beta) / \sigma_{d + \beta}} / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} e^{(d(x, c_i) + \beta) / \sigma_{d + \beta}} / (|X| - |C|)} \\ 
= 
\frac{\sum_{i=1}^{|C|}|C_i|e^{d(c_i, c) / \sigma_{d}} / (|C| - 1)}{\sum_{i=1}^{|C|} \sum_{x \in C_i} e^{d(x, c_i)/ \sigma_{d}} / (|X| - |C|)} \cdot \frac{e^\beta}{e^\beta} = CH_1(C, X, d).
\end{multline*}
Therefore, $CH_1$ is Shift Invariant.
This makes $CH_2$ and $CH_3$, which are functions that gets $CH_1$ as input, Shift Invariant. Then, as $CH_{btwn}$ is an aggregation of $CH_3$, due to Theorem 9, $CH_{btwn}$ is Shift Invariance. \hfill $\Box$






% \textbf{Theorem 1.} \textit{For $N$-dimensional Gaussian distribution $G(0, I)$, the mean of Euclidean distances of vectors randomly sampled from the distribution grows in $O(\sqrt{N})$ while standard deviation stays constant (i.e., grows in $O(1)$).}

% \textit{Proof. } For vectors $x_i \sim G(0, I)$ and $y_i \sim G(0, I)$, $(x_1 - x_2) \sim G(0, \sqrt{2}I)$. Thus, $\| x_1 - x_2 \|^2 / 2 \sim \chi^2_N$, which leads to $\| x_1 - x_2 \| / (\sqrt{2}) \sim \chi_N$. Here, mean $\mu$ and standard deviation $s$ of $\chi_N$ is determined as:
% \[ 
% \mu: \sqrt{2}\frac{\Gamma((N+1)/2)}{\Gamma(N/2)}, s: \sqrt{N - \mu^2} \:\: \cite{abell99ap}.
% \]
% Now, by applying S\'andor's inequality \cite{sandor06rgmia}
% $\sqrt{x} \leq \Gamma(X + 1) / \Gamma(X + 1/2) \leq \sqrt{x+ 1/2}$, which is a stronger version of Gautschi's inequality \cite{kershaw83mc},  we know that $\mu$ satisfies
% \[
% \sqrt{2} \cdot \sqrt{\frac{N-1}{2}} \leq \mu \leq \sqrt{2} \cdot\sqrt{\frac{N}{2}}.
% \]
% As  $\sqrt{(N-1)/2} = O(\sqrt{N})$ and $\sqrt{(N)/2} = O(\sqrt{N})$, $\mu=O(\sqrt{N})$.
% The above inequality also leads to the inequality $0 \leq s = \sqrt{N - \mu^2} \leq 1$, which implies $s = O(1)$.

% Hence, the theorem is true. \hfill $\Box$


==> appendices/C_basis_dataset.tex <==

\section{Basis datasets Used in Validity Analysis}

\label{app:basis}

Following figure depicts a subset of basis dataset consists of two 2D Gaussian distribution used in validity analysis. We diversified the dataset in perspective of dimensionality, scale, number of points, and randomness to verify whether our between-dataset IVM satisfies the axioms.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/basis.pdf} 
    \caption{\mac{Do not use yellow with white background. Use blue/red instead} Subset of 1,000 2D basis datasets used in validity analysis, where each consists of two Gaussian distributions (left) and the dimension-augmented version of the datasets (right). For each 2D dataset, we randomized two distributions' size, variance, and a distance between them. To augment the dimensionality without disturbing the original cluster structure, we added Gaussian noise while maintain the variance of the noise smaller than the original distributions' variance. In this figure, only 3D augmented data was expressed, but data with a higher dimension was also created. }
    \label{fig:validity_data}
\end{figure}

==> appendices/D_experiment_setting.tex <==
\section{Detailed Settings in Between-dataset Rank Correlation Analysis}

\label{app:detail_btw}

\textbf{Classifiers settings. } As aforementioned, for consistency, we exploited the setting of Rodr\'iguez et al. \cite{rodriques18kbs}. The hyperparameters are set as follows:
\begin{itemize}
    \item \textbf{Support Vector Machine} (SVM): We used C-support vector classification model with default hyperparameter setting provided by \texttt{sklearn} \cite{pedregosa11jmlr}. 
    \item \textbf{$k$-Nearest Neighbor} ($k$NN): We used $k=1$, and for all other parameters, we used default setting of \texttt{sklearn}. \mac{That is not really good use of KNN, several values should be tried}
    \item \textbf{Multilayer Perceptron} (MLP): We used 500 epochs, learning rate of 0.3, and momentum of 0.2. We used single hidden layer, where the size of the hidden layer is determined as the half the sum of dimension and number of classes. All other parameters are set to the default provided by \texttt{sklearn}. 
    \item \textbf{Naive Bayesian networks} (NB): We used default parameter setting provided by \texttt{sklearn}.
    \item \textbf{Random forest} (RF): We used RF classifier consists of 100 trees with max depth of 10. Remaining parameters are set to the default of \texttt{sklearn}.
    \item \textbf{Logistic regression} (LR): We used 100 iterations. All remaining parameters are set to the default of \texttt{sklearn}.
    \item \textbf{Linear discriminant analysis} (LDA): We used least squares solution solver, and all other parameters are set to the default provided by \texttt{sklearn}.
\end{itemize}

We conducted 5-fold cross validation for each classifier, and used a mean value as a final classification score for a dataset. For the ensemble of classifiers, we used the max combination of the classifiers (i.e., chose the highest score among the classifiers).\mac{we miss the end of the story. we rank the scatterplot based on this classification score.}

\mac{For all supervised techniques, there should be a  grid search over the meta-parameters. you shall use Auto-ML or similar package for Python (pick the one with the most technique and the most recent): https://automl.github.io/auto-sklearn/master/ 
https://hyperopt.github.io/hyperopt-sklearn/
https://auto.gluon.ai/stable/tutorials/tabular\_prediction/tabular-quickstart.html
}

\textbf{Settings for computing ground-truth data-CLM.}
We used \texttt{sklearn} implementation for DBSCAN, $K$-Means, Birch, Agglomerative clustering, \texttt{sklearn-extra} implementation for $K$-Medoids, and \texttt{pyclustering} implementation for $X$-Means. For HDBSCAN, we used the implementation of McInnes et al. \cite{mcinnes17oss}. 
To find the best hyperparameter setting for each clustering technique, we used Bayesian optimization \cite{snoek12neurips} implementation provided by Nogueira \cite{nogueira14github}. For each clustering techniques, we performed five random exploration and 25 steps of optimization, which are the defaults of the implementation. 
The bounds of each technique's hyperparameter is set as follows:
\begin{itemize}
    \item \textbf{DBSCAN}
    \begin{itemize}
        \item \texttt{epsilon}: [0.01, 1.0]
        \item \texttt{min\_samples}: [1, 10]
    \end{itemize}
    \item \textbf{HDBSCAN}
    \begin{itemize}
        \item \texttt{epsilon}: [0.01, 1.0]
        \item \texttt{min\_samples}: [1, 10]
        \item \texttt{min\_cluster\_size}: [2, 50]
    \end{itemize}
    \item \textbf{\textit{K}-Means}
    \begin{itemize}
        \item $K$ (numver of clusters): [2, (number of classes of data) $\cdot$ 3]
    \end{itemize}
    \item \textbf{\textit{K}-Medoids}
    \begin{itemize}
        \item $K$: [2, (number of classes of data) $\cdot$ 3]
    \end{itemize}
    \item \textbf{\textit{X}-Means}
    \begin{itemize}
        \item \texttt{kmax}: [2, 50]
        \item \texttt{tolerance}: [0.01, 1.0]
    \end{itemize}
    \item \textbf{Birch}
    \begin{itemize}
        \item \texttt{threshold}: [0.1, 1.0]
        \item \texttt{branching\_factor}: [10, 100]
    \end{itemize}
    \item \textbf{Agglomerative Clustering}
    \begin{itemize}
        \item number of clusters: [2, (number of classes of data) $\cdot$ 3]
    \end{itemize}
\end{itemize}
After finding the best hyperparameter setting of a clustering technique for a given datasets, we ran the technique 20 times with same setting and report the average value as the final score. 


\newpage

==> appendices/E_datasets.tex <==
\section{Datasets used in Rank Correlation Analyses}

\label{app:datasets}

\mac{Add another table (two columns) showing all datasets ranked by their decreasing value of CHbtwn, together with the CHbtwn score}

\begin{table}[H]
    
  \caption{Real-World Datasets used in Between-dataset and Within-Dataset Rank Correlation Analyses }
  \label{dataset-table}
  \centering \small
  \begin{tabular}{lllll}
    \toprule
    Dataset & Objects & Features & Classes & Reference \\
    \midrule
        Birds Bones and Living Habits & 413 & 10 & 6 & Kaggle~\cite{kaggle} \\
        Cardiovascular Study Dataset & 2,927 & 15 & 2 & Kaggle \\
        Credit Risk Classification Dataset & 976 & 11 & 2 & Kaggle \\
        Customer Classification & 1,000 & 11 & 4 & Kaggle \\
        Fraud detection bank dataset 20K records binary & 20,468 & 112 & 2 & Kaggle \\
        Heart Attack Analysis \& Prediction Dataset & 303 & 13 & 2 & Kaggle \\
        League of Legends Diamond Games & 48,651 & 17 & 2 & Kaggle \\
        Microbes Dataset & 30,527 & 24 & 10 & Kaggle \\
        Mobile Price Classification & 2,000 & 20 & 4 & Kaggle \\
        Music Genre Classification & 1,000 & 26 & 10 & Kaggle \\
        Orbit Classification For Prediction / NASA & 1,748 & 11 & 6 & Kaggle \\ % Orbit NASA
        Paris Housing Classification & 10,000 & 17 & 2 & Kaggle \\
        pH-recognition & 653 & 3 & 15 & Kaggle \\
        Rice Seed Dataset (Gonen\&Jasmine) & 18,185 & 10 & 2 & Kaggle \\ % Rice type classification
        Siberian Weather Stats & 1,439 & 11 & 9 & Kaggle \\
        Smoker Condition & 1,012 & 7 & 2 & Kaggle \\
        Water Quality & 2,011 & 9 & 2 & Kaggle \\
        Wine Customer Segmentation & 178 & 13 & 3 & Kaggle \\ % Wine Customer
        
        banknote authentication & 1,372 & 4 & 2 & UCI ML Repo~\cite{asuncion07uci} \\
        Breast Cancer Wisconsin (Prognostic) & 569 & 30 & 2 & UCI ML Repo \\
        Breast Tissue & 106 & 9 & 6 & UCI ML Repo \\
        CNAE-9 & 1,080 & 856 & 9 & UCI ML Repo \\
        Dermatology & 358 & 34 & 6 & UCI ML Repo \\
        Echocardiogram & 61 & 10 & 2 & UCI ML Repo \\
        Ecoli & 336 & 7 & 8 & UCI ML Repo \\
        Glass Identification & 214 & 9 & 6 & UCI ML Repo \\
        Harberman's Survival & 306 & 3 & 2 & UCI ML Repo \\
        Hepatitis & 80 & 19 & 2 & UCI ML Repo \\
        Image Segmentation & 210 & 19 & 7 & UCI ML Repo \\
        Ionosphere & 351 & 34 & 2 & UCI ML Repo \\
        Iris & 150 & 4 & 3 & UCI ML Repo \\
        Letter Recognition & 20,000 & 16 & 26 & UCI ML Repo \\
        MAGIC Gamma Telescope & 19,020 & 10 & 2 & UCI ML Repo \\
        Optical Recognition of Handwritten Digits & 3,823 & 64 & 10 & UCI ML Repo \\
        Pen-Based Recognition of Handwritten Digits & 7,494 & 16 & 10 & UCI ML Repo \\
        Planning Relax & 182 & 12 & 2 & UCI ML Repo \\
        SECOM & 1,567 & 590 & 2 & UCI ML Repo \\ % secom
        Spambase & 4,601 & 57 & 2 & UCI ML Repo \\
        SPECTF Heart & 80 & 44 & 2 & UCI ML Repo \\
        Statlog (German Credit Data) & 1,000 & 24 & 2 & UCI ML Repo \\ % German Credit Numeric
        Statlog (Image Segmentation) & 2,310 & 19 & 7 & UCI ML Repo \\
        Taiwanese Bankruptcy Prediction Data Set & 6,819 & 95 & 2 & UCI ML Repo \\ % Company Bankruptcy Prediction
        Wine & 178 & 13 & 3 & UCI ML Repo \\
        Yeast & 1,484 & 8 & 10 & UCI ML Repo \\
        Zoo & 101 & 16 & 7 & UCI ML Repo \\
        
        Blood Transfusion Service Center & 748 & 4 & 2 & Yeh et al.~\cite{yeh2009knowledge} \\
        Boston & 154 & 13 & 3 & Sedlmair et al.~\cite{sedlmair2012taxonomy} \\
        Breast Cancer Coimbra & 116 & 9 & 2 & Patrício et al.~\cite{patricio2018using} \\
        Breast Cancer Wisconsin (Original) & 683 & 9 & 2 & Wolberg et al.~\cite{wolberg1990multisurface} \\
        CIFAR10 & 3,250 & 1,024 & 10 & Krizhevsky et al.~\cite{krizhevsky2009learning} \\ % cifar10
        Classification in asteroseismology & 1,001 & 3 & 2 & Hon et al.~\cite{hon2017deep} \\
        COIL20 & 1,440 & 400 & 20 & Nene et al.~\cite{nene20columbia} \\ % coil20
        Crowdsourced Mapping & 10,545 & 28 & 6 & Johnson et al.~\cite{johnson2016integrating} \\
        Date Fruit Datasets & 898 & 34 & 7 & Koklu et al.~\cite{koklu2021classification} \\
        Diabetic Retinopathy Debrecen Data Set & 1,151 & 19 & 2 & Antal et al.~\cite{antal2014ensemble} \\
        Dry Bean Dataset & 13,611 & 16 & 7 & Koklu et al.~\cite{koklu2020multiclass} \\
        Durum Wheat Features & 9,000 & 236 & 3 & Kaya et al.~\cite{kaya2019towards} \\
    \bottomrule
    
  \end{tabular}
  
\end{table}


\begin{table}[H]
  \label{dataset-table2}
  \centering \small
  \begin{tabular}{lllll}
    \toprule
    Dataset & Objects & Features & Classes & Reference \\
    \midrule
        Epileptic Seizure Recognition & 5,750 & 178 & 5 & Andrzejak et al.~\cite{andrzejak2001indications} \\ % epileptic
        ExtyaleB & 319 & 30 & 5 & Georghiades et al.~\cite{georghiades2001few} \\
        Fashion-MNIST & 3,000 & 784 & 10 & Xiao et al.~\cite{xiao2017fashion} \\ % fashion mnist
        Fetal Health Classification & 2,126 & 21 & 3 & Ayres-de-Campos et al.~\cite{ayres2000sisporto} \\
        Flickr Material Database & 997 & 1,536 & 10 & Sharan et al.~\cite{sharan2009material} \\ % fmd
        HAR & 735 & 561 & 6 & Anguita et al.~\cite{anguita2012human} \\ % har
        Hate Speech & 3,221 & 100 & 3 & Davidson et al.~\cite{davidson2017automated} \\ % hatespeech
        Heart Disease & 297 & 13 & 5 & Detrano et al.~\cite{detrano1989international} \\
        HIVA & 3,076 & 1,617 & 2 & Guyon et al.~\cite{guyon2007agnostic} \\ % hiva
        HTRU2 & 17,898 & 8 & 2 & Lyon et al.~\cite{lyon2016fifty} \\ % Pulsar Dataset HTRU2
        Human Stress Detection & 2,001 & 3 & 3 & Rachakonda et al.~\cite{rachakonda2019stress} \\ % Stress Detection
        IMDB & 3,250 & 700 & 2 & Maas et al.~\cite{maas2011learning} \\ % imdb
        Insurance Company Benchmark  & 5,822 & 85 & 2 & Putten et al.~\cite{van2004bias} \\ % The Insurance Company (TIC) Benchmark
        Labeled Faces in the Wild & 2,200 & 5,828 & 2 & Huang et al.~\cite{huang2008labeled} \\
        Mammographic Mass & 830 & 5 & 2 & Elter et al.~\cite{elter2007prediction} \\
        Mnist64 & 1,082 & 64 & 6 &  Xia et al.~\cite{xia22tvcg} \\
        Olivetti faces dataset & 400 & 4,096 & 40 & AT\&T Lab. Cambridge~\cite{atntlab} \\
        Parkinsons & 195 & 22 & 2 & Little et al.~\cite{little2007exploiting} \\ % Parkinsons Disease Dataset
        Patient Treatment Classification & 4,412 & 10 & 2 & Mujiono Sadikin~\cite{sadikin2020} \\
        Pima Indians Diabetes Database & 768 & 8 & 2 & Smith et al.~\cite{smith1988using} \\
        Pistachio Dataset & 2,148 & 28 & 2 & Ozkan et al.~\cite{ozkan2021classification} \\
        Pumpkin Seeds Dataset & 2,500 & 12 & 2 & Koklu et al.~\cite{koklu2021use} \\
        Raisin Dataset & 900 & 7 & 2 & Cinar et al.~\cite{ccinar2020classification} \\
        Rice Dataset Cammeo and Osmancik & 3,810 & 7 & 2 & Cinar et al.~\cite{cinar2019classification} \\
        seeds & 210 & 7 & 3 & Charytanowicz et al.~\cite{charytanowicz2010complete} \\
        Seismic Bumps & 646 & 24 & 2 & Sikora et al.~\cite{sikora2010application} \\ % seismic
        Sentiment Labeled Sentences & 2,748 & 200 & 2 & Kotzias et al.~\cite{kotzias2015group} \\ % sentiment
        SkillCraft1 Master Table Dataset & 3,338 & 18 & 7 & Thompson et al.~\cite{thompson2013video} \\ % SkillCraft-StarCraft
        SMS Spam Collection & 835 & 500 & 2 & Almeida et al.~\cite{almeida2011contributions} \\ % sms
        Street View House Numbers & 732 & 1,024 & 10 & Netzer et al.~\cite{netzer2011reading} \\ % svhn
        student grade pass or fail & 395 & 29 & 2 & Cortez et al.~\cite{cortez2008using} \\
        Turkish Music Emotion Dataset & 400 & 50 & 4 & Er et al.~\cite{er2019music} \\
        User Knowledge Modeling & 258 & 5 & 4 & Kahraman et al.~\cite{kahraman2013development} \\
        Weather & 365 & 192 & 7 & Ventocilla et al.~\cite{ventocilla2020comparative} \\
        Website Phishing & 1,353 & 9 & 3 & Abdelhamid et al.~\cite{abdelhamid2014phishing} \\
        Wilt & 4,339 & 5 & 2 & Johnson et al.~\cite{johnson2013hybrid} \\
        Wine Quality & 4,898 & 11 & 7 & Cortez et al.~\cite{cortez2009modeling} \\
        Wireless Indoor Localization & 2,000 & 7 & 4 & Rohra et al.~\cite{rohra2017user} \\
        World12d & 150 & 12 & 5 & Sedlmair et al.~\cite{sedlmair2012taxonomy} \\
    \bottomrule
    
  \end{tabular}
  
\end{table}

==> appendices/F_time_analysis.tex <==
\section{Running Time Comparison}

\label{app:time}

==> appendices/_deprecated_B_internal_measures.tex <==
\section{Detailed Explanation of Internal Measures}
\label{app:im}

\subsection{Internal Clustering Validation}
\label{sec:icv}

As clustering algorithm's goal is to maximize distinction between clusters and similarity within a cluster, most internal measures are designed to measure clusterings based on two criteria: separability and compactness \cite{liu10idcm, tan05idm, zhao02cikm, rendon11ac}. While separability denotes the degree to which clusters are apart from other clusters, compactness represents closeness of the points within a cluster. 
Most measures are defined as the \textit{Ratio} (e.g., Calinski-Harabasz \cite{calinski74cis}, Xie-Beni \cite{xie91tpami}), \textit{Difference }(e.g., Silhouette \cite{rousseeuw87jcam}), or \textit{Sum }(e.g., $S\_Dbw$ \cite{halkidi01icdm}, $CVNN$ \cite{liu13tc}) of two criteria. Here, we list nine widely used internal measures surveyed by Liu et al. \cite{liu10idcm} and Xiong and Li. \cite{xiong13cvm}, and and organize them in three categories. In \autoref{sec:clustgen}, we demonstrate how these measures are generalized to clusterness measures. Note that we only considered monotonic measures, where optimal clustering is determined as the one with maximum or minimum score, instead of the shift point (i.e., the elbow) \cite{halkidi01jiis} which requires subjective determination to be judged. Exact definitions of the measures can be found in Table XXX.




\begin{table}
  \caption{Definition of commonly used internal measures (\autoref{sec:icv}) and their characteristics. Note that there is no fixed range for $SD$ and $CVNN$, as their range depends on normalization factors, which are determined based on currently compared clusterings.}
  \label{sample-table}
  \centering \small
  \begin{tabular}{cclcc}
    \toprule
    Type & Symbol & Definition & Optimal & Range \\
    \midrule
     Ratio & $CH$  & $\frac{\sum_i|C_i|d^2(c_i, c) / (NC-1)}{\sum_i \sum_{x\in C_i} d^2(x, c_i) / (|D| - NC)}$  & max & $(0, \infty)$ \\
     Ratio  & $I$  & $(\frac{1}{NC} \cdot \frac{\sum_{x \in D} d(x, c)}{\sum_i \sum_{x \in C_i} d(x, c_i)} \cdot \max_{i, j} d(c_i, c_j)) ^ p$ ($p=2$ for default)   & max & $(0, \infty)$ \\
     Ratio & $D$  &  $\frac{\min_{i,j} \min_{x \in C_i, y \in C_j} d(x, y)}{\max_k \max_{x, y \in C_k} d(x, y)}$ & max & $(0, \infty)$  \\
    Ratio & $XB$ &  $ \frac{\sum_i \sum_{x \in C_i} d^2(x, c_i)}{|D| \cdot \min_{i, j \neq i} d^2(c_i, c_j)}$ & min & $(0,\infty)$ \\
     Ratio & $DB$   & $\frac{1}{NC} \cdot \sum_i \max_{j\neq i}\frac{\sum_{k =\{i, j\}}(\frac{1}{|C_k|}\sum_{x \in C_k} d(x, c_k))}{d(c_i, c_j)} $ & min & $(0, \infty)$  \\
    Sum & $S\_Dbw$  & $Scat + Dens\_bw$ & min & (0, 2)\\
        &           & $Scat = \frac{1}{NC} \sum_i \| \sigma(C_i) \| / \| \sigma(D) \|$ & &  \\
        &           & $Dens\_bw = \frac{1}{NC \cdot (NC-1)} (\sum_{i, j \neq i} \frac{density(u_{ij})}{\max(density(c_i), density(c_j))})$ &  & \\
    Sum  & $SD$ & $\alpha \cdot Scat + Dis$ & min & - \\
       &        & $Dis = \frac{\max_{i, j} d(c_i, c_j)}{\min_{i, j} d(c_i, c_j)} \cdot \sum_i (\sum_j d(c_i, c_j))^{-1}$ & & \\
    Sum & $CVNN$   & $Sep(k) / \max_{NC} + Com / \max_{NC}$ & min & - \\ 
    & & $Sep = \max_i(\frac{1}{|C_i|} \sum_{j=1, 2, \cdots, |C_i|} \frac{q_j}{k}) $ & & \\
    & & $Com = \sum_i(\frac{2}{|C_i| \cdot (|C_i| -1 ) } \sum_{x,y \in C_i} d(x,y))$ & & \\
    Diff  & $SC$ & $\frac{1}{NC} \cdot \sum_i [\frac{1}{|C_i|} \cdot\sum_{x \in C_i} \frac{b(x) - a(x)}{\max(b(x), a(x))}]$ & min & (-1, 1) \\ 
       &  & $a(x) = \frac{1}{|C_i| - 1} \sum_{y \in C_i, y \neq x} d(x, y)$ & & \\ 
       &  & $b(x) = \min_{j \neq i} (\frac{1}{|C_j|} \sum_{y \in C_j} d(x,y))$ & &\\
    \bottomrule
    \addlinespace[0.115cm]
    \multicolumn{5}{l}{
        \footnotesize
        $D$: dataset; $C_i$: $i$-th cluster; $c / c_i$: centroid of dataset / $i$-th cluster; $NC$: number of clusters;  
    } \\
    \multicolumn{5}{l}{
        \footnotesize
         $d(x, y)$: distances between points $x$ and $y$; $v(C)$: varaince vector of $C$; $\| v \| = \sqrt{v^T \cdot v}$;
    } \\
    \multicolumn{5}{l}{
        \footnotesize
         $u_{ij}$: midpoint of $c_i$ and $c_j$; $density(u_{ij}) = \sum_{x \in D} f(x, u_{ij})$, $density(c_i) = \sum_{x \in C_i} f(x, c_i)$;
    } \\ 
    \multicolumn{5}{l}{
        \footnotesize
         $f(x, c) = 0$ if $d(x, c) > \frac{1}{NC} \sqrt{\sum_i\| \sigma(C_i) \|}$ and else 1; $k$: number of considered nearest neighbors
    } \\ 
    \multicolumn{5}{l}{
        \footnotesize
         $q_j$: number of $C_i$'s $j$-th point's nearest neighbors that are not belong to $C_i$
    } \\ 
  \end{tabular}
  
\end{table}



\textit{Ratio. } 
Calinski-Harabasz index ($CH$) \cite{calinski74cis} evaluates compactness as a sum of squared distances each each point to its cluster centroid, and separability as a sum of squared distances of each cluster centroids to the global centroid of entire dataset. 
I Index ($I$) \cite{maulik02tpami} computes compactness as a ratio of sum of distances of points to its cluster centroid to the sum of points to the global centroid. Separability is defined as a sum of pairwise distances between centroids. 
In Dunn's index ($D$) \cite{dunn74joc}, compactness is  maximum intra-cluster distance and separability is minimum inter-cluster distance. 
Xie-Beni Index ($XB$) \cite{xie91tpami} uses same definition for compactness with $CH$, while defining separability as minimum pairwise distances between centroids.
For Davies-Bouldin Index ($DB$), the similarity of two clusters are first defined where compactness is a sum of distances of points to their cluster centroid, and separability is a distance between centroids. Then, final score is computed as an average of the score assigned to each cluster; each cluster's score corresponds to the max similarity with among the ones with other clusters. 
These measures are defined in a form of $Score = (a \cdot Separability) / (b \cdot Compactness)$ ($CH$, $I$, $D$) or its inverse ($XB$, $DB$). While the higher value implies better clustering in the former, lower value implies better clustering in the latter. 

\textit{Summation. }
S\_Dbw Index ($S\_Dbw$) \cite{halkidi01icdm} evaluates compactness as a ratio of the average of cluster variance to the entire variance of the dataset. Separability instead takes the concept of density; for each pair of clusters, separation is defined as a ratio of density around midpoint of the cluster centroid to the density around centroids. SD Index ($SD$) \cite{halkidi00pkdd}  shares the definition of compactness with $S\_Dbw$, while utilizes the sum of cluster centroids to represent separation. Clustering Validation index based on Nearest Neighbors ($CVNN$)  \cite{liu13tc} compute separability as an average ratio of each points' nearest neighbors belonging to the same cluster to the total number of nearest neighbors. Compactness is computed as an average intra-cluster pairwise distances.
These three measures simply compute the final score as a sum of separability and compactness. However, as the range of separability and compactness can vary, the measures often requires additional adjustment. For example, in $SD$, additional weighting factor is multiplied to compactness to balance it with separability. In contrast, $CVNN$ normalizes both separability and compactness to the maximum separability and compactness computed among all clusterings that are currently compared. 

\textit{Difference. }
Silhouette coefficient ($SC$) \cite{rousseeuw87jcam} quantifies average difference between mean intra-cluster distance (compactness) and the mean nearest-cluster distance (separability) for every point. The optimal clustering is determined as the one having the max index. 


As internal validation measures are naturally designed to find optimal clustering , most of them cannot be used across datasets. 
However, at least $S$ have been used across dataset; it is widely used to evaluate DR by quantifying the extent to which a cluster structure of the original space are well represented in the embeddings \cite{joia11tvcg, fadel15neurocomp}. Still, this use case is about comparing datasets with identical dimension, number of points and clusters. 
Our generalization instead allows the measure to be used across arbitrary datasets, thus enables various useful application scenarios.

